Roadmap for the international, accelerator-based neutrino programme

In line with its terms of reference the ICFA Neutrino Panel has developed a roadmapfor the international, accelerator-based neutrino programme. A "roadmap discussion document" was presented in May 2016 taking into account the peer-group-consultation described in the Panel's initial report. The "roadmap discussion document" was used to solicit feedback from the neutrino community---and more broadly, the particle- and astroparticle-physics communities---and the various stakeholders in the programme. The roadmap, the conclusions and recommendations presented in this document take into account the comments received following the publication of the roadmap discussion document. With its roadmap the Panel documents the approved objectives and milestones of the experiments that are presently in operation or under construction. Approval, construction and exploitation milestones are presented for experiments that are being considered for approval. The timetable proposed by the proponents is presented for experiments that are not yet being considered formally for approval. Based on this information, the evolution of the precision with which the critical parameters governinger the neutrino are known has been evaluated. Branch or decision points have been identified based on the anticipated evolution in precision. The branch or decision points have in turn been used to identify desirable timelines for the neutrino-nucleus cross section and hadro-production measurements that are required to maximise the integrated scientific output of the programme. The branch points have also been used to identify the timeline for the R&D required to take the programme beyond the horizon of the next generation of experiments. The theory and phenomenology programme, including nuclear theory, required to ensure that maximum benefit is derived from the experimental programme is also discussed.

==> 08-Conc-n-rec/08-01-CnR.tex <==
\stepcounter{nuPanel-RM-Conc-Sect}

\noindent
\framebox[\textwidth][l]{
  \parbox[c]{0.98\linewidth}{
    \begin{description}
      \stepcounter{nuPanel-RM-Conc-Sect-Conc}
      \item[\arabic{nuPanel-RM-Conc-Sect}.\arabic{nuPanel-RM-Conc-Sect-Conc}:]
        The neutrino has a tiny mass, much smaller than any other
        fundamental fermion, and its type, or ``flavour'', changes as
        it propagates through space and time.
        These properties imply the existence of new phenomena not
        described by the Standard Model of particle physics and may
        have profound consequences for our understanding of the
        Universe. 
        The tiny neutrino mass seems likely to be related to phenomena
        that occur at very high energy scales, well beyond the reach
        of the present or proposed colliding-beam facilities.
        The study of the neutrino is therefore the study of physics
        beyond the Standard Model and a fundamentally important
        component of the particle-physics programme.
      \stepcounter{nuPanel-RM-Conc-Sect-Conc}
      \item[\arabic{nuPanel-RM-Conc-Sect}.\arabic{nuPanel-RM-Conc-Sect-Conc}:]
        The accelerator-based neutrino programme is global in
        scope, engagement and intellectual contribution.
        Continued and enhanced cooperation in a coherent global
        programme will maximise the impact of each individual
        contribution and of the programme as a whole.
        \begin{description}
          \stepcounter{nuPanel-RM-Conc-Sect-Rec}
          \item[\color{BlueViolet} Recommendation \arabic{nuPanel-RM-Conc-Sect}.\arabic{nuPanel-RM-Conc-Sect-Rec}:]
            \textbf{\color{BlueViolet} The present roadmap discussion
              document should be completed through discussion with the
              stakeholders.  
              The roadmap should then be revised and updated at
              appropriate intervals.
            }
        \end{description}
      \stepcounter{nuPanel-RM-Conc-Sect-Conc}
      \item[\arabic{nuPanel-RM-Conc-Sect}.\arabic{nuPanel-RM-Conc-Sect-Conc}:]
        By collating data from a number of sources the Panel has
        gained a partial understanding of the strength of the global
        accelerator-based neutrino community.
        Accurate, up-to-date, consistent and complete census data
        for the global accelerator-based neutrino community will be
        valuable in planning the development of the programme.
        \begin{description}
          \stepcounter{nuPanel-RM-Conc-Sect-Rec}
          \item[\color{BlueViolet} Recommendation \arabic{nuPanel-RM-Conc-Sect}.\arabic{nuPanel-RM-Conc-Sect-Rec}:]
            \textbf{\color{BlueViolet} ICFA should support the Panel
              in its efforts to work with the stakeholders to gather
              the necessary census data as part of the consultation
              process that will follow the completion of this roadmap
              discussion document. 
            }
        \end{description}
    \end{description}
  }
}

